Coordinating Planning and Tracking in Layered Control Policies via Actor-Critic Learning

We propose a reinforcement learning (RL)-based algorithm to jointly train (1) a trajectory planner and (2) a tracking controller in a layered control architecture. Our algorithm arises naturally from a rewrite of the underlying optimal control problem that lends itself to an actor-critic learning approach. By explicitly learning a \textit{dual} network to coordinate the interaction between the planning and tracking layers, we demonstrate the ability to achieve an effective consensus between the two components, leading to an interpretable policy. We theoretically prove that our algorithm converges to the optimal dual network in the Linear Quadratic Regulator (LQR) setting and empirically validate its applicability to nonlinear systems through simulation experiments on a unicycle model.

==> tex/41-AnalysisBackup.tex <==
\section{Analysis for Linear Quadratic Regulator}\label{sec:analysis}
In this section, we focus on the case of noiseless linear quadratic regulator (LQR) problems and show that our method for updating the dual network can learn to predict the optimal dual variable if we solve the tracking problem well enough. We choose to focus on the dual update as the problem of learning the optimal tracking controller and its value function has been studied extensively both empirically and theoretically. In what follows, we define the problem we analyze, and first show that dual network updates of the form \eqref{eq:dual-update} can converge to the optimal dual map if one can perfectly solve the planning \eqref{eq:upper-level-opt} and tracking problem \eqref{eq:lower-level-opt}. We then end with a perturbation result that shows that the algorithm will converge to the vicinity of the optimal dual variable if we learn to solve the tracking and planning problem well enough.

For the rest of this section, we consider the instantiation of problem \eqref{eq:redundant-prob} where
\begin{equation}\label{eq:quadratic-cost}
\begin{gathered}
    \mathcal{C}(r) = \sum_{t=0}^{T} r_t^\top Q r_t =: r^\top \mathcal{Q} r,\\
    \mathcal{D}(u) = \sum_{t=0}^{T-1} u_t^\top R u_t =: u^\top \mathcal{R} u,
\end{gathered}
\end{equation}

where we define $\mathcal{Q} = I_{T} \otimes Q$ and $\mathcal{R} = I_{T-1} \otimes R$. The dynamics is given as
\begin{equation}\label{eq:linear-dynamics}
    x_{t+1} = f(x_t, u_t) = A x_t + B u_t.
\end{equation}
We consider the unconstrained case where $\mathcal{X} = \R^{d_x}$, and the initial condition $\xi$ is sampled i.i.d. from the standard normal distribution $\mathcal{N}(0, I)$.

\subsection{With Optimal Tracking}
We begin by noting that, in this case, the optimal dual variable\footnote{If not further specified, when we refer to $\nu$ or the dual variable, we mean the dual variable associated with the constraint $r=x$ in problem \eqref{eq:redundant-prob}} $\nu^*$ is a linear function of the initial condition $x_0$. (See Lemma \ref{lem:dual-existence} in Appendix \ref{sec:appendix-proof-opt}.) We thus parametrize our dual network as a linear map
\begin{equation}\label{eq:lqr-dual-pred}
    v_\theta(\xi) = \Theta \xi.
\end{equation}
We first consider the case where we can solve the planning \eqref{eq:upper-level-opt} and tracking problem \eqref{eq:lower-level-opt} optimally, i.e., that we consider the following update rule. In each iteration, we first sample a minibatch of initial conditions $\{\xi^{(k)}_i\}_{i=1}^{B} \overset{i.i.d.}{\sim} \mathcal{N}(0, I)$, and use the current $\Theta^{(k)}$ to predict the optimal dual variable
\begin{equation*}
    \hat{v}^{(k+1)}_i = v_{\theta^{(k)}}(\xi_i) = \Theta^{(k)} \xi_i.
\end{equation*}
For each initial condition, we solve the trajectory optimization problem
\begin{equation}\label{eq:opt-traj-opt-update}
    r^{(k+1)}_i = \text{argmin}_r r^\top Q r + p^*(r + \hat{v}_i^{(k+1)}; \xi),
\end{equation}
where $p^*$ is the optimal value of the tracking problem
\begin{equation}\label{eq:opt-tracking-update}
\begin{aligned}
        x^{(k+1)}_i, u^{(k+1)}_i = \text{argmin}_{x, u}& u^\top R u + \frac{\rho}{2} \lVert r^{(k+1)}_i + \hat{v}^{(k+1)}_i - x\rVert\\
        \text{s.t.}\quad& x_{t+1} = Ax_t + Bu_t,\\
        &x_0 = \xi.
\end{aligned}
\end{equation}
After solving \eqref{eq:opt-tracking-update}, we update the dual network parameter $\Theta$ as
\begin{equation}\label{eq:lqr-dual-update}
    \begin{aligned}    
    \Theta^{(k+1)} &= \Theta^{(k)} + \\
    &\quad \eta \nabla_\Theta \left( \sum_{i=1}^{B} \frac{1}{B} \left(r^{(k+1)}_i - x^{(k+1)_i}\right)^\top v_{\Theta^{(k+1)}}(\xi_i)\right)\\
    %
    &=  \Theta^{(k)} + \eta\sum_{i=1}^{B} \frac{1}{B} \left(r^{(k+1)}_i - x^{(k+1)_i}\right) \xi_i^\top
    \end{aligned}
\end{equation}
For this update rule where we solve both trajectory planning and tracking perfectly as in \eqref{eq:opt-traj-opt-update} and \eqref{eq:opt-tracking-update}, we show that the following is true.
\begin{theorem}\label{thm:opt-tracking}
    Consider the cost functions \eqref{eq:quadratic-cost} and dynamics \eqref{eq:linear-dynamics}. Given any $\Theta^{(0)}$, by repeatedly applying the update rules \eqref{eq:lqr-dual-pred}-\eqref{eq:lqr-dual-update}, the iterate $\Theta^{(k)}$ converges to the optimal $\Theta^*$ exponentially. Specifically, we have that there exists step size $\eta > 0$, mini-batch size $B$ such that
    \begin{equation*}
        \mathbb{E} \norm{\Theta^{(k)} - \Theta^{*}}_2 \leq \gamma^k \mathbb{E} \norm{\Theta^{(0)} - \Theta^{*}}_2,
    \end{equation*}
    where $0< \gamma < 1$.
\end{theorem}
\begin{proof}
    See Appendix \ref{sec:appendix-proof-opt}.
\end{proof}

\subsection{With Suboptimal Tracking}\label{sec:analysis-subopt}
The analysis in the previous subsection is achieved only when one learns the tracking controller $\pi^l$ and its value function $p^\pi$ perfectly. In this section, we consider the case where the learned tracking controller is not optimal. In this case, we show that if the learned tracking controller is close to optimal, one can guarantee that the dual map $\Theta$ will converge to a small ball around $\Theta^*$, where the radius of the ball depends on the error of the learned tracking controller.

In this setting, we know that the optimal tracking controller is a linear function and its value function is a quadratic function of the augmented state. Thus, we consider perturbations in this form. Specifically, we consider a case where the $r$-update \eqref{eq:opt-traj-opt-update} is perturbed by an inaccuracy in the learned value function $p^*$ as
\begin{equation}\label{eq:r-update-perturb}
    \hat{p}(\tilde{r}, \xi) = p^*(\tilde{r}; \xi) + (\tilde{r} - F\xi) \Delta_P (\tilde{r} - F\xi)
\end{equation},
which parallels the quadratic form of $p^*$. For the $u$-update \eqref{eq:opt-tracking-update}, we consider a perturbation and $u$-update that is linear in the reference and the initial state
\begin{equation}\label{eq:u-update-perturb}
    \hat{u}(\tilde{r}, \xi) = u^*(\tilde{r}, \xi) + \Delta_{u,r}\tilde{r} + \Delta_{u, \xi} \xi
\end{equation}
where $u^*$ denotes the $u$ solution of \eqref{eq:opt-tracking-update}. Here, $\Delta_P, \Delta_{u,r}, \Delta_{u, x_0}$ are matrices of appropriate dimensions and represent the inaccuracies in the learning controller and the estimate of its value function.

\begin{theorem} \label{thm:subopt-tracking}(informal)
Consider the cost functions \eqref{eq:quadratic-cost} and dynamics \eqref{eq:linear-dynamics}.Consider the update rules \eqref{eq:lqr-dual-pred}-\eqref{eq:lqr-dual-update} with the perturbations \eqref{eq:r-update-perturb} and \eqref{eq:u-update-perturb}. Denote the size of the perturbations as $\epsilon_P = \norm{\Delta_P}, \epsilon_{u,r} = \norm{\Delta_{u,r}}, \epsilon_{u,\xi} = \norm{\Delta_{u,\xi}}$. Given any $\Theta^{(0)}$, if the perturbations $\epsilon_P, \epsilon_{u,r}$ are small enough, there exist step size $\eta$ and batch size $B$ such that
\begin{multline*}
    \E \norm{\Theta^{(k)} - \Theta^*} \leq \\
    \gamma^k \E \norm{\Theta^{(0)} - \Theta^*} + \frac{1-\rho^k}{1-\rho} e(\epsilon_P, \epsilon_{u,r}, \epsilon_{u,\xi}),
\end{multline*}
where $0 < \gamma < 1$.
\end{theorem}
\begin{proof}
    See Appendix \ref{sec:appendix-proof-subopt} for a formal statement and proof.
\end{proof}
In the next section, we validate the theoretical guarantees with numerical experiments.

==> tex/Other.tex <==
\section{Related Work}
Summarize works in the areas of
\begin{enumerate}
    \item Hierarchical reinforcement learning, specifically goal-conditioned reinforcement learning. \cite{vezhnevets2017feudal}
    \item Existing hierarchical actor-critic methods \cite{levy2017learning, roder2020curious}
    \item Bi-level planning \cite{silver2023predicate}
    \item Layering in control \cite{srikanthan2023data, matni2016theory, chiang2007layering}
\end{enumerate}

\subsection{Hierarchical Reinforcement Learning}
The reinforcement learning community has long studied the idea of hierarchy as a way to improve exploration and planning over long horizons \cite{dayan1992feudal, pateria2021hierarchical}. Our approach is closely related to the idea of \textit{goal-conditioned} reinforcement learning \cite{kulkarni2016hierarchical, levy2017learning, nachum2018data, vezhnevets2017feudal}. In this framework, an upper-level agent specifies goals for the lower level agent to execute. The upper-level agent is usually trained on the upper-level reward specified by the actual objective while the lower-level agent is trained on a parameterized reward that seeks to capture the degree to which it completes the goal set by the high-level agent. Most of these approaches also incorporate the idea of temporal abstraction, i.e., the goal set by the meta-controller will persist for several steps on the time scale of the low-level controller.

\subsubsection{Tricks}
Something else to note is that \textbf{directional} goals are usually used instead of absolute goals \cite{vezhnevets2017feudal, nachum2018data}. This is potentially better because the low level agent can "reuse" its past experience much better.

A lot of these approaches do \textbf{hindsight relabeling} of various sorts \cite{nachum2018data, levy2017learning}.

\cite{vezhnevets2017feudal} uses a linear combination of environment reward and parametrized intrinsic reward for the low level (instead of just using the parametrized reward).

Goals do not have to be specified in the original state-space, but can be instead mapped onto a low-dimensional latent space \cite{vezhnevets2017feudal, nachum2018near}. This significantly increases scalability if the observation space is high-dimensional (eg. image). However, to do this in a principled manner requires careful thinking about the information lost in the process of encoding the observation into the latent space. This can be partially overcome by using a principled loss for learning the encoder and modifying the lower-level reward function \cite{nachum2018near}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5methods section%%%%%%%%%%%%%%%%%%%%%%%%
We apply the actor-critic algorithm to both the upper layer trajectory generation problem and the lower layer tracking problem. Overall, there are a total four components involved:
\begin{itemize}
    \item the upper-level actor $\pi^h(x_0; \nu)$ and critic $Q^h(x_0, r; \nu)$, and
    \item the lower-level actor $\pi^l(x, \tilde{r})$ and critic $Q^l(x, \tilde{r}, u)$.
\end{itemize}
A careful examination quickly reveals that $Q^h$ is determined by the lower-level components, namely
\begin{equation*}
\begin{aligned}
        Q^h(x_0, r; \nu) &= \mathcal{C}(r) + J(x_0, r; \nu)\\
        &= \mathcal{C}(r) + Q^l(x_0, r - \nu, \pi^l(x_0, r-\nu)).
\end{aligned}
\end{equation*}
Thus, our goal is to learn the three functions $\pi^h$, $\pi^l$, and $Q^l$. The overall idea is to parameterize all three functions are neural networks and learn the low-level components via standard actor-critic algorithm, while updating the upper-level $\pi^h$ occasionally during the training. In what follows, we first review some basics of actor-critic learning, and then show how to adapt the setup to our particular problem.

Following this intuition, one way to solve the primal minimization step is to
\begin{enumerate}
    \item find a good tracking controller $\pi^l(x, r)$ for any initial state $x$ and reference trajectory $r$.
    \item estimate its cost-to-go $V^l(x, r)$ under the stage tracking cost $\lVert \tilde{r} - x \rVert_2^2 + \mathcal{D}(u)$.
    \item Find the optimal value of the $(x,u)$-optimization problem
    $$J(x_0, r; \nu) = V^l(x_0, r - \nu).$$
    \item the trajectory generator $\pi^h(x_0; \nu)$ is found by solving the optimization problem $$\pi^j(x_0; \nu) = \text{argmin}_r\;\; \mathcal{C}(r) + J(x_0, r; \nu).$$
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{enumerate}
    \item The fact that the planner can learn to exploit a fixed low-level controller is a very interesting one. This suggests two things. (1) Folding the low-level controller into the environment and directly optimizing the planner without explicit consideration of the low-level controller is an approach that almost artificially injects fragility to your system. This is because your planner can learn to exploit your low-level controller in ways you never would understand. (I doubt one would be able to draw the trajectories generated by the learned planner.) (2) This also brings in a very interesting game-theoretic aspect to this problem. We almost want the low-level controller to play a Nash equilibrium strategy in the sense that we do not want the high-level planner to be able to exploit it. (3) Surya: This is actually reminiscent of RL algorithms exploiting idiosyncrasies of sim.  Optimizers are just too good at exploiting any loopholes.
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Unlike the general nonlinear case, we can get away with learning just a $Q$-function for the tracking problem, as it is well-known that the value function for an LQR-tracking problem is quadratic, and the greedy action can be found easily by solving a quadratic program. Further, we consider the unconstrained case where a closed-form solution for the optimal tracking problem can be obtained. There are thus two components that we would like to learn: 1) an action-value function $Q(s, a)$ for the tracking problem, and 2) a map from the initial state $x_0$ to a prediction of the optimal dual variable $v$. Specifically, we will leverage the known information of the problem and parameterize the $Q$ function as a quadratic function and the dual map as a linear map, i.e., that
\begin{gather*}
    Q_{\phi}(s, a) = \begin{bmatrix} s^\top & a^\top \end{bmatrix} \Phi \begin{bmatrix} s \\ a \end{bmatrix}
\end{gather*}
For the analysis, we assume that we will first learn a tracking controller to convergence, and then use the learned tracking controller to fit the dual map using our proposed algorithm in a dual ascent fashion.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The Deep Deterministic Policy Gradient (DDPG) algorithm \cite{lillicrap2015continuous} is developed to handle the setting where one would like to use actor-critic methods for a deterministic policy that is parameterized as a neural network. It uses the deterministic policy gradient theorem shown in \cite{silver2014deterministic} in combination with many engineering tricks to stabilize the training. Specifically, they
\begin{enumerate}
    \item use Q-learning along with replay buffer for the critic
    \item use a target network for both policy and critic to stabilize training (at the expense of slowing down learning)
    \item use batch normalization to make sure that the range of all the features are standardized
    \item exploration with additive noise
\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Our algorithm thus becomes an iterative process between these three steps:
\begin{equation}\label{eq:update-rule}
    \begin{aligned}
            \hat{v}^{(k+1)}_i &= v_{\theta^{(k)}}(\xi_i), \xi_i \sim \mathcal{N}(0,1)\\
    r^{(k+1)}_i &= \text{argmin}_r r^\top Q r + p^*(r + \hat{v}_i^{(k+1)})\\
    x^{(k+1)}_i, u^{(k+1)}_i &= \text{argmin}_{x, u} u^\top R u + \frac{\rho}{2} \lVert r^{(k+1)}_i + \hat{v}^{(k+1)}_i - x\rVert\\
    &\text{s.t.}\;\quad x_{t+1} = Ax_t + Bu_t,\quad x_0 = \xi\\
    \theta^{(k+1)} &= \theta^{(k)} + \eta \nabla_\theta \sum_{i=1}^{B} \frac{1}{B} \left(r^{(k+1)}_i - x^{(k+1)_i}\right)^\top\hat{v}^{(k+1)}_i
    \end{aligned}
\end{equation}
